A game of life with dormancy

The factors contributing to the persistence and stability of life are fundamental for understanding complex living systems. Organisms are commonly challenged by harsh and fluctuating environments that are suboptimal for growth and reproduction, which can lead to extinction. Species often contend with unfavorable and noisy conditions by entering a reversible state of reduced metabolic activity, a phenomenon known as dormancy. Here, we develop Spore Life, a model to investigate the effects of dormancy on population dynamics. It is based on Conway's Game of Life, a deterministic cellular automaton where simple rules govern the metabolic state of an individual based on the metabolic state of its neighbors. For individuals that would otherwise die, Spore Life provides a refuge in the form of an inactive state. These dormant individuals (spores) can resuscitate when local conditions improve. The model includes a parameter alpha that controls the survival probability of spores, interpolating between Game of Life (alpha = 0) and Spore Life (alpha = 1), while capturing stochastic dynamics in the intermediate regime (0 < alpha < 1). In addition to identifying the emergence of unique periodic configurations, we find that spore survival increases the average number of active individuals and buffers populations from extinction. Contrary to expectations, the stabilization of the population is not the result of a large and long-lived seed bank. Instead, the demographic patterns in Spore Life only require a small number of resuscitation events. Our approach yields novel insight into what is minimally required for the emergence of complex behaviors associated with dormancy and the seed banks that they generate.

==> older/method_older.tex <==
We propose a cellular automaton model that includes dormancy. Under variation of a single parameter, $\alpha$, the
model transitions between the well-known Conway's Game of Life (GoL) in the limit $\alpha \to 0$ and our modified model,
subsequently called Spore Life (SL) in the limit $\alpha \to 1$. For the intermediate parameter regime, $\alpha \in (0, 1)$,
the model is stochastic, where the exact value of $\alpha$ could be interpreted to encode the difference between shallow and deep dormancy.

\paragraph{Conway's Game of Life}
The model is given as a cellular automaton defined on a $\ell\times \ell$ grid. We start with the usual update rules of
Conway's Game of Life and later present our modification. In GoL, each cell can have one of two states
$S\in \{ \mathrm{ALIVE}, \mathrm{DEAD} \}\equiv \{\mathrm{A},\mathrm{D}\}$. Initially the grid is seeded randomly with some ALIVE cells, where
a cell is ALIVE with probability $q$. The grid advances in discretized time steps $t\in \mathbb{N}_0$, where the
initial condition is present at time step $t = 0$. In each time step the grid is updated according to the following
update rules:
\begin{enumerate}
    \item A DEAD cell is reborn if it has exactly 3 ALIVE neighbors (reproduction),
    \item an ALIVE cell with less than 2 ALIVE neighbors dies (loneliness),
    \item an ALIVE cell with 2 to 3 ALIVE neighbors stays ALIVE,
    \item an ALIVE cell with more than 3 ALIVE neighbors dies (overpopulation).
\end{enumerate}
The rules are summarized in Fig.~\ref{fig:rule-tables}~(top)

\paragraph{Spore Life}
We include dormancy by adding a third state, SPORE, such that a cell can be in either of three states,
$S \in \{ \mathrm{ALIVE}, \mathrm{SPORE}, \mathrm{DEAD} \}\equiv \{\mathrm{A}, \mathrm{S}, \mathrm{D}\}$.
In each time step the grid is updated according to the following modified update rules:
\begin{enumerate}
    \item A DEAD cell is reborn if it has exactly 3 ALIVE neighbors (reproduction),
    \item an ALIVE cell with exactly 1 ALIVE neighbor becomes a SPORE (scarce resources, dormancy),
    \item a SPORE cell with 2 or 3 ALIVE neighbors becomes ALIVE (wake up),
    \item a SPORE cell less than 2 or more than 3 ALIVE neighbors stays a SPORE,
    \item an ALIVE cell with 2 to 3 ALIVE neighbors stays ALIVE,
    \item an ALIVE cell with exactly 0 ALIVE neighbors dies (loneliness),
    \item an ALIVE cell with more than 3 ALIVE neighbors dies (overpopulation).
\end{enumerate}
In addition to that a parameter $\alpha\in[0, 1]$ is introduced. After each iteration every SPORE dies with
the probability $(1-\alpha)$, which ensures that the model retains the Markov property.
The parameter $\alpha$ may therefore be interpreted as the endurance of SPOREs in unclear conditions
which could be related to shallow dormancy ($\alpha$ small) or deep dormancy ($\alpha$ large). The rules are summarized in
Fig.~\ref{fig:rule-tables}~(middle).
Note, that for $\alpha = 0$ we recover the rule table of Game of Life, considering the fact that new SPORE cells immediately
die.

\paragraph{Shallow vs. Deep Dormancy}
A cell in a shallowly dormant state will not be able to retain dormancy for long, but will eventually die. On the other hand,
a cell in a deeply dormant state may still wake up after a long period of staying dormant.

This difference is captured by our model. For small values of $\alpha$, SPOREs die relatively quickly, where dormancy is
impossible in the limit $\alpha \to 0$. On the other hand, for large $\alpha$ SPOREs can remain in a state of dormancy
for a long time (see Fig.~\ref{fig:spore-lifetime-distr}) before dying, and can stay dormant for eternity in the limit
$\alpha \to 1$.
